The One RING: a Robotic Indoor Navigation Generalist

Modern robots vary significantly in shape, size, and sensor configurations used to perceive and interact with their environments. However, most navigation policies are embodiment-specific--a policy trained on one robot typically fails to generalize to another, even with minor changes in body size or camera viewpoint. As custom hardware becomes increasingly common, there is a growing need for a single policy that generalizes across embodiments, eliminating the need to retrain for each specific robot. In this paper, we introduce RING (Robotic Indoor Navigation Generalist), an embodiment-agnostic policy that turns any mobile robot into an effective indoor semantic navigator. Trained entirely in simulation, RING leverages large-scale randomization over robot embodiments to enable robust generalization to many real-world platforms. To support this, we augment the AI2-THOR simulator to instantiate robots with controllable configurations, varying in body size, rotation pivot point, and camera parameters. On the visual object-goal navigation task, RING achieves strong cross-embodiment (XE) generalization--72.1% average success rate across five simulated embodiments (a 16.7% absolute improvement on the Chores-S benchmark) and 78.9% across four real-world platforms, including Stretch RE-1, LoCoBot, and Unitree Go1--matching or even surpassing embodiment-specific policies. We further deploy RING on the RB-Y1 wheeled humanoid in a real-world kitchen environment, showcasing its out-of-the-box potential for mobile manipulation platforms. (Project website: https://one-ring-policy.allen.ai)

==> figs/human_eval_layout.tex <==
% \begin{figure}[!ht]
% 	\centering
% 	\includegraphics[width=0.8\columnwidth]{figs/human_eval_layout.pdf}
% 	\caption{
% \textbf{Real-world test scene for human evaluation}. Three different target objects include (\includegraphics[height=3mm]{figs/apple.png} \texttt{Apple}, \includegraphics[height=3mm]{figs/leaf.png} \texttt{Houseplant}, \includegraphics[height=3mm]{figs/mug.png} \texttt{Mug}). The red arrow in the bottom left corner is the starting location.}
% 	\label{fig:human_eval_layout}
% \end{figure}





% \begin{table}[t]
% \begin{minipage}{.45\linewidth}
%   \centering
% 	\includegraphics[width=1\columnwidth]{figs/human_evaluators.pdf}
% 	\caption{\footnotesize{
% \textbf{Human Participants for Navigation Assitance}. Our five human participants have different height and different camera-holding poses, resulting in different sensory observations (details about human participants in Table~\ref{tab:human_spec}).}}
% 	\label{fig:human_evaluator}
% \end{minipage}%
% \hspace{0.5cm}
% \begin{minipage}{.50\linewidth}
%   \centering
  
%   \vspace{-2mm}
%   \tiny
%   \setlength{\tabcolsep}{1pt}
%   \renewcommand{\arraystretch}{1.2}
% 	\centering
% 	\includegraphics[width=0.8\columnwidth]{figs/human_eval_layout.pdf}
% 	\caption{
% \footnotesize{\textbf{Real-world test scene for human evaluation}. Three different target objects include (\includegraphics[height=3mm]{figs/apple.png} \texttt{Apple}, \includegraphics[height=3mm]{figs/leaf.png} \texttt{Houseplant}, \includegraphics[height=3mm]{figs/mug.png} \texttt{Mug}). The red arrow in the bottom left corner is the starting location.}}
% 	\label{fig:human_eval_layout}
% \end{minipage}
% \vspace{-6mm}
% \end{table}





\begin{table}[t]
\begin{minipage}{.6\linewidth}
  \centering
  \includegraphics[width=0.9\columnwidth]{figs/human_eval_pdf.pdf}
  % \vspace{-2mm}
  \caption{\footnotesize{\textbf{Human Trajectories}. Two sample trajectories from two individuals navigating to a houseplant and an apple using \model.}}
	\label{fig:human_eval}
\normalsize
\end{minipage}%
\hspace{0.2cm}
\begin{minipage}{.4\linewidth}
  \centering
  
  \vspace{-2mm}
  \tiny
  \setlength{\tabcolsep}{1pt}
  \renewcommand{\arraystretch}{1.2}
	\centering
	\includegraphics[width=0.8\columnwidth]{figs/human_eval_layout_pdf.pdf}
	\caption{
\footnotesize{\textbf{Real-world test scene for human evaluation}. Three different target objects include (\includegraphics[height=3mm]{figs/apple.png} \texttt{Apple}, \includegraphics[height=3mm]{figs/leaf.png} \texttt{Houseplant}, \includegraphics[height=3mm]{figs/mug.png} \texttt{Mug}). The red arrow in the bottom left corner is the starting location.}}
	\label{fig:human_eval_layout}
\end{minipage}
\vspace{-6mm}
\end{table}

==> tables/human_results.tex <==
\begin{table}[t]
\centering
% \small
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccccccc}


\multirow{2}{*}{Model} & \multirow{2}{*}{Train Embodiment} & \multirow{2}{*}{Object} & \multicolumn{5}{c}{Human Participants} & \\
\cmidrule(r){4-8} %\cmidrule(r){4} \cmidrule(r){5}
& & & \multicolumn{1}{c}{\textbf{H1}}  & \multicolumn{1}{c}{\textbf{H2}} & \multicolumn{1}{c}{\textbf{H3}}& \multicolumn{1}{c}{\textbf{H4}}& \multicolumn{1}{c}{\textbf{H5}} & Average \\

\midrule
\multirow{3}{*}{\textsc{FLaRE}~\cite{hu2024flare}} & \multirow{3}{*}{Stretch RE-1} & \includegraphics[height=3mm]{figs/apple.png} & \textcolor{OliveGreen}{\cmark} & \textcolor{BrickRed}{\xmark} & \textcolor{BrickRed}{\xmark} & \textcolor{BrickRed}{\xmark} & \textcolor{BrickRed}{\xmark} & \multirow{3}{*}{40.0\%} \\ 
&  & \includegraphics[height=3mm]{figs/leaf.png} & \textcolor{BrickRed}{\xmark} & \textcolor{OliveGreen}{\cmark} & \textcolor{OliveGreen}{\cmark} & \textcolor{OliveGreen}{\cmark} & \textcolor{OliveGreen}{\cmark} & \\ 
&  & \includegraphics[height=3mm]{figs/mug.png} & \textcolor{BrickRed}{\xmark} & \textcolor{BrickRed}{\xmark} & \textcolor{BrickRed}{\xmark} & \textcolor{BrickRed}{\xmark} & \textcolor{OliveGreen}{\cmark}  & \\ 

\midrule
\multirow{3}{*}{\modelzeroshot} & \multirow{3}{*}{\model-Random} & \includegraphics[height=3mm]{figs/apple.png} & \textcolor{OliveGreen}{\cmark} & \textcolor{BrickRed}{\xmark} & \textcolor{BrickRed}{\xmark} & \textcolor{BrickRed}{\xmark} & \textcolor{OliveGreen}{\cmark} & \multirow{3}{*}{\textbf{73.3\%}} \\
& & \includegraphics[height=3mm]{figs/leaf.png} & \textcolor{OliveGreen}{\cmark} & \textcolor{OliveGreen}{\cmark} & \textcolor{OliveGreen}{\cmark} & \textcolor{OliveGreen}{\cmark} & \textcolor{OliveGreen}{\cmark} & \\
& & \includegraphics[height=3mm]{figs/mug.png} & \textcolor{BrickRed}{\xmark} & \textcolor{OliveGreen}{\cmark} & \textcolor{OliveGreen}{\cmark} & \textcolor{OliveGreen}{\cmark} & \textcolor{OliveGreen}{\cmark} & \\

% \bottomrule
\end{tabular}
}
% \normalsize
\caption{\textbf{Human Evaluation.} Five individuals navigate to 3 different objects (\includegraphics[height=3mm]{figs/apple.png} \texttt{Apple}, \includegraphics[height=3mm]{figs/leaf.png} \texttt{Houseplant}, \includegraphics[height=3mm]{figs/mug.png} \texttt{Mug}) following the policy's output actions on their phones in a kitchen area (example trajectories in Fig.~\ref{fig:human_eval}). \modelzeroshot shows much better generalization to human embodiment than the FLaRE baseline trained on Stretch RE-1.} 
\label{tab:humans}
\vspace{-.5em}
\end{table}

==> tables/nearest_neighbors_locobot.tex <==
\setlength{\tabcolsep}{2pt}
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.0}
\scriptsize
\begin{tabular}{lllllll}
& & \multicolumn{5}{c}{Nearest Neighbors} \\
\cmidrule(r){3-7} 
& \textbf{Locobot} & N1 & N2 & N3 & N4 & N5 \\
\hline 
Camera Position (x) (meters)& 0 & -0.09 & 0.12 & 0.03 & $-0.06$ & -0.1 \\
Camera Position (y) (meters)& 0.87 & 1.01 & 0.81 & 0.39 & 0.85 & 0.42 \\
Camera Position (z) (meters)& 0 & -0.1 & -0.05 & -0.1 & -0.02 & 0.09 \\
Camera Pitch (degrees) & 0 & 0 & 0 & -1 & 0 & 1 \\
Camera Yaw (degrees) & 0 & 0 & 0 & 0 & 0 & 0 \\
Vertical FoV (degrees)& 42 & 45 & 44 & 42 & 45 & 45 \\
RGB Resolution (H) & 224 & 224 & 224 & 224 & 224 & 224 \\
RGB Resolution (Y) & 396 & 396 & 394 & 394 & 392 & 392 \\
Rotation Center (x) (meters)& 0 & 0.04 & 0.1 & 0.1 & -0.02 & -0.15 \\
Rotation Center (z)  (meters)& 0 & -0.13 & 0 & 0.13 & 0.02 & -0.12 \\
Collider Size (x) (meters)& 0.35 & 0.27 & 0.36 & 0.37 & 0.27 & 0.42 \\
Collider Size (y) (meters)& 0.89 & 1.28 & 1.23 & 0.86 & 1.46 & 0.59 \\
Collider Size (z) (meters)scale z & 0.4 & 0.43 & 0.23 & 0.36 & 0.36 & 0.45 \\
\hline
distance & - & 0.18 & 0.22 & 0.34 & 0.41 & 0.42 \\
\hline
\end{tabular}
\normalsize
\caption{\footnotesize{Five Nearest Neighbor Embodiments for LoCoBot in Training Data.} }
\label{tab:nn_locobot}
% \vspace{-1.5em}
\end{table}
